Offline Reinforcement Learning with Domain-Unlabeled Data

Offline reinforcement learning (RL) is vital in areas where active data collection is expensive or infeasible, such as robotics or healthcare. In the real world, offline datasets often involve multiple domains that share the same state and action spaces but have distinct dynamics, and only a small fraction of samples are clearly labeled as belonging to the target domain we are interested in. For example, in robotics, precise system identification may only have been performed for part of the deployments. To address this challenge, we consider Positive-Unlabeled Offline RL (PUORL), a novel offline RL setting in which we have a small amount of labeled target-domain data and a large amount of domain-unlabeled data from multiple domains, including the target domain. For PUORL, we propose a plug-and-play approach that leverages positive-unlabeled (PU) learning to train a domain classifier. The classifier then extracts target-domain samples from the domain-unlabeled data, augmenting the scarce target-domain data. Empirical results on a modified version of the D4RL benchmark demonstrate the effectiveness of our method: even when only 1 to 3 percent of the dataset is domain-labeled, our approach accurately identifies target-domain samples and achieves high performance, even under substantial dynamics shift. Our plug-and-play algorithm seamlessly integrates PU learning with existing offline RL pipelines, enabling effective multi-domain data utilization in scenarios where comprehensive domain labeling is prohibitive.

==> sec/checklist.tex <==
\paragraph{Format}

\begin{itemize}
    \item \textbf{Figure}:
    \begin{itemize}
        \item Are the figure num., caption below the figure?
        \item Are figures cited before or in the same page as them?
    \end{itemize}
    \item \textbf{Table}: Are they cited before or in the same page as them?
    \item \textbf{Equation}:
    \begin{itemize}
        \item Are they cited by eqref?
        \item With not cited one is defined with*?
    \end{itemize}
    \item \textbf{Section}: Are they precisely cited?
    \item \textbf{Contributions}: Are all the contributions well supported??
\end{itemize}

\paragraph{Handling of previous review of RLC 2024}
\begin{itemize}
    \item In the preliminaries, a dataset is defined as a 4-tuple but in Problem Formulation a +1 is added to each data instance in
    without explanation.
    \textcolor{blue}{I removed the +1 from the definition of the dataset.}
    \item The introduction’s explanation of “domain” (specifically the first para) could be clearer and more direct. It assumes familiarity with the term’s application in RL without providing a clear definition. The use of the highly specific example might not adequately illustrate a “domain”’s broader relevance. A more straightforward definition / explanation could also improve the understanding of the problem’s motivation and challenges. Moreover, ‘domain’ is not officially defined in the preliminaries. It is unclear how Positive-unlabeled learning relates to domains until the Problem Formulation in which the reader must infer a domain from the Definition of Positive-unlabeled offline RL.
    \textcolor{blue}{I explicitly explain the domain in the introduction. Also, I defined the domain in the preliminaries.}
    \item The authors attempt to maintain statistical integrity by applying this test (along with Welch’s t-test and the Mann-Whitney U test), but it is ultimately limited due to the small sample size (5 seeds). Shapiro-Wilk's effectiveness is specifically limited in this case because it may lack the power to detect deviations from normality.
    \textcolor{blue}{I increased the number of seeds to 10.}
    \item The approach is effective within a framework where the unlabelled data distribution is limited to two domains. Hence the scope of applying such a method is very constrained. The author did not offer additional evidence to justify this constraint. I do not find the method to be scaleable to practical applications involving more than two distributions.
    \textcolor{blue}{We no longer consider only two domains. We consider multiple domains.}
    \textcolor{blue}{I added the experiments on the modified version of the D4RL benchmark with dynamics shift, where only $1\%$--$3\%$ of the data are domain-labeled. This result shows that our method is effective even when only a tiny fraction of labeled positive samples are available.}
    \item I find the comparison of baselines in the paper to be unfair. It is obvious that offline RL would struggle with limited data (e.g., Only-labeled-positive utilizing only 3% of the data) or with a mixture of positive and negative samples (Using-All). Comparing "Dynamic-Aware Reward Augmentation" as a baseline seems unreasonable. Instead, the baseline should be compared with other methods that propose training under unlabeled datasets.
    While the paper relies on empirical evidence, it does not provide code to reproduce the results.
    \textcolor{blue}{I added more clear explanation of why we compare with the baselines.}


\end{itemize}
